Certifiably Adversarially Robust Detection of Out-of-Distribution Data

Deep neural networks are known to be overconfident when applied to out-of-distribution (OOD) inputs which clearly do not belong to any class. This is a problem in safety-critical applications since a reliable assessment of the uncertainty of a classifier is a key property, allowing the system to trigger human intervention or to transfer into a safe state. In this paper, we aim for certifiable worst case guarantees for OOD detection by enforcing not only low confidence at the OOD point but also in an $l_\infty$-ball around it. For this purpose, we use interval bound propagation (IBP) to upper bound the maximal confidence in the $l_\infty$-ball and minimize this upper bound during training time. We show that non-trivial bounds on the confidence for OOD data generalizing beyond the OOD dataset seen at training time are possible. Moreover, in contrast to certified adversarial robustness which typically comes with significant loss in prediction performance, certified guarantees for worst case OOD detection are possible without much loss in accuracy.

==> sections/calibration.tex <==
\section{Calibration of classifiers} \label{section:calibration}
The model being calibrated means that for an outside observer knowing not the input but only the prediction of the model, the likelihood of the input belonging to a certain class equals that predicted probability:
\begin{align}
    \Prob \left(y \mid \f(x) \right) = p_{y}(x) .
\end{align}

Standard real world classifiers, however, tend to be quite badly calibrated \cite{GuoEtAl2017}.
For one, overfitting to a training set in general leads to overconfident predictions, but simply re-scaling the outputs is not sufficient to achieve good calibration.

==> sections/provable_classidiers.tex <==
\section{A review of provably robust classifiers} \label{section:ibp}
\iffalse
Interval bound propagation is a method for DNNs proposed by \citep{gowal2018effectiveness} that provides entrywise lower and upper bounds for each layer's feature vector within an $\epsilon$-sized $\ell_\infty$-Ball around an input point $x$.
Concretely, the bounds of  $\pm \epsilon$ are propagated forward through each individual layer. 
Notably for a layer that -- like convolutional layers -- can be written in affine form $z_{n-1} \mapsto W_n \cdot z_{n-1} + b_n$, this forward propagation works for the upper bound with
\begin{align}
     \overline{z_n}^\epsilon = \max(W_n, 0) \cdot  \overline{z_{n-1}}^\epsilon + \min(W_n, 0)  \cdot \underline{z_{n-1}}_\epsilon
\end{align} 
 and conversely for the lower bound with 
\begin{align}
    \underline{z_n}_\epsilon = \min(W_n, 0) \cdot \overline{z_{n-1}}^\epsilon + \max(W_n, 0) \cdot \underline{z_{n-1}}_\epsilon \ ,
\end{align}
where the $\min$ and $\max$ expressions are to be understood for each individual entry of the matrix.
Note that $\overline{z_0}^\epsilon = x + \epsilon$ and $\underline{z_0}_\epsilon = x - \epsilon$, with $\epsilon$ added to / subtracted from each component, while each subsequent activation vector has component-specific bounds.
ReLU functions are directly applied to the bounds.
The idea behind the original IBP's last layer elision is that one can obtain tighter bounds by regarding the final affine layer more concretely, a thought that we slightly modify in Equation \eqref{eq:logitud} to fit our objective.

The calculations involved in this forward propagation of the bounds are of similar functional nature as the standard forward pass and thus can be easily back-propagated.
This results in additional forward and backward pass times of roughly twice those of the standard model.
\fi

\cite{HeiAnd2017}
Other methods like \cite{WonKol2018}, \cite{MirGehVec2018} and \cite{WangMixtrain} also give very tight robustness guarantees.
The main advantage -- that is also crucial for our goal -- of IBP is its practicality for direct and fast optimization of good guarantees....[]
Note that verification techniques do not in general transfer from one method that a model was optimized for to another method for obtaining guarantees, although [] reports some working results...
The recently published CROWN-IBP \cite{zhang2020towards} combines IBP and relaxation based methods.

Downsides of IBP based methods, which our models mostly share, are for one a limited model depth and unclear compatibility with certain deep learning methods, lowering the classification accuracy achievable by the architecture.
Furthermore, hyperparameters and training schedules have to be chosen very carefully, and a higher number of training epochs compared to standard classifiers is often necessary.
In addition, provably robust classification normally has a severe negative impact on clean test accuracy, an issue that the GOOD method does not experience in a major form.




==> tables/table_auc_old.tex <==
\begin{table*}[t]
\caption{\textbf{OLD} AUROC statistics obtained by thresholding confidence of in-distribution predictions and out-distribution predictions, pgd-adversarials and ibp-guarantees. The models used are 02-03-10-01-08 and 02-02-21-31-52}

\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{clc|ccc|ccc}
\toprule
In dataset & Out dataset      & Predictions     & $\epsilon_{test}$ & Advers. & Guarant.  & $\epsilon_{test}$ & Advers. & Guarant.     \\
\midrule
\multirow{5}{*}{MNIST}      
& Uniform Noise         & 100.0 & \multirow{5}{*}{0.1} 
                                   & 100.0 & 100.0 & \multirow{5}{*}{0.4}             
                                                      & 100.0 & 100.0     \\
& FashionMNIST          & 100.0 &  & 100.0 & 85.8  & & 100.0 & 35.0     \\
& EMNIST Letters        & 98.7  &  & 90.8  & 30.2  & & 98.7  & 00.2     \\
& GrayCIFAR-10              & 100.0 &  & 100.0 & 99.9  & & 100.0 & 81.6     \\
& 80M Tiny Images       & 100.0 &  & 100.0 & 99.3  & & 100.0 & 79.9     \\
\midrule
\multirow{5}{*}{CIFAR10}      
& Uniform Noise     & 98.6 & \multirow{4}{*}{0.01}             
                                           & X  & 99.5 & \multirow{4}{*}{8/255} 
                                                            & 98.6     & 78.1     \\
& SVHN              & 70.3  & & X     & 33.7 &              & 28.5     & 27.0      \\
& CIFAR-100         & 74.9  & & X     & 46.7 &              & 41.3     & 38.8      \\
& 80M Tiny Images   & 81.8  & & X     & 61.4 &              & 54.0     & 51.1      \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


==> tables/table_conf_histograms.tex <==
\begin{table*}[t]
\caption{Confidences on the CIFAR-10 in-distribution and on several OOD datasets.
}
\label{table:conf_histograms}
\setlength\tabcolsep{.5pt} % default value: 6pt
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\makebox[\textwidth][c]{
\begin{tabularx}{1.4\textwidth}{CCCCCC}
Model   &   CIFAR10  &    CIFAR-100   &   SVHN    & LSUN CR   & Uniform   \\
Plain &
    \includegraphics[width=1.0\linewidth]{images/histograms/Plain_CIFAR10_in_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/Plain_CIFAR100_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/Plain_SVHN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/Plain_LSUN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/Plain_Noise_Dataset_noise_uniform_pred_confidences_hist.png} \\
CEDA &
    \includegraphics[width=1.0\linewidth]{images/histograms/CEDA_CIFAR10_in_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/CEDA_CIFAR100_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/CEDA_SVHN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/CEDA_LSUN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/CEDA_Noise_Dataset_noise_uniform_pred_confidences_hist.png} \\
OE &
    \includegraphics[width=1.0\linewidth]{images/histograms/OE_CIFAR10_in_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/OE_CIFAR100_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/OE_SVHN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/OE_LSUN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/OE_Noise_Dataset_noise_uniform_pred_confidences_hist.png} \\
ACET &
    \includegraphics[width=1.0\linewidth]{images/histograms/ACET_CIFAR10_in_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/ACET_CIFAR100_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/ACET_SVHN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/ACET_LSUN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/ACET_Noise_Dataset_noise_uniform_pred_confidences_hist.png} \\
GOOD\textsubscript{0} &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD0_CIFAR10_in_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD0_CIFAR100_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD0_SVHN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD0_LSUN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD0_Noise_Dataset_noise_uniform_pred_confidences_hist.png} \\
GOOD\textsubscript{20} &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD20_CIFAR10_in_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD20_CIFAR100_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD20_SVHN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD20_LSUN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD20_Noise_Dataset_noise_uniform_pred_confidences_hist.png} \\
\end{tabularx}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

\begin{table*}[t]
\caption{Confidences on the CIFAR-10 in-distribution and on several OOD datasets.
}
\label{table:conf_histograms_cont}
\setlength\tabcolsep{.5pt} % default value: 6pt
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\makebox[\textwidth][c]{
\begin{tabularx}{1.4\textwidth}{CCCCCC}
Model   &   CIFAR10  &    CIFAR-100   &   SVHN    & LSUN CR   & Uniform   \\
GOOD\textsubscript{40} &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD40_CIFAR10_in_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD40_CIFAR100_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD40_SVHN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD40_LSUN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD40_Noise_Dataset_noise_uniform_pred_confidences_hist.png} \\
GOOD\textsubscript{60} &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD60_CIFAR10_in_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD60_CIFAR100_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD60_SVHN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD60_LSUN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD60_Noise_Dataset_noise_uniform_pred_confidences_hist.png} \\
GOOD\textsubscript{80} &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD80_CIFAR10_in_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD80_CIFAR100_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD80_SVHN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD80_LSUN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD80_Noise_Dataset_noise_uniform_pred_confidences_hist.png} \\
GOOD\textsubscript{90} &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD90_CIFAR10_in_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD90_CIFAR100_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD90_SVHN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD90_LSUN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD90_Noise_Dataset_noise_uniform_pred_confidences_hist.png} \\
GOOD\textsubscript{95} &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD95_CIFAR10_in_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD95_CIFAR100_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD95_SVHN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD95_LSUN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD95_Noise_Dataset_noise_uniform_pred_confidences_hist.png} \\
GOOD\textsubscript{100} &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD100_CIFAR10_in_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD100_CIFAR100_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD100_SVHN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD100_LSUN_pred_confidences_hist.png}   &
    \includegraphics[width=1.0\linewidth]{images/histograms/GOOD100_Noise_Dataset_noise_uniform_pred_confidences_hist.png} \\
\end{tabularx}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


==> tables/table_prelim.tex <==
\begin{table*}[t]
\caption{eps=0.01. 1000 samples. all models RN20, eexcept CEDA CE Tiny which is RN32.}
\setlength\tabcolsep{.5pt} % default value: 6pt
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\makebox[\textwidth][c]{
\begin{tabularx}{1.3\textwidth}{lc|CC|CC|CC|CC|CC|CC|CC|CC|CC}
\toprule
Model & Acc. & CIFAR10 & P/G & SVHN & P/G & uniform & P/G & low freq & P/G & CIFAR100 & P/G & TinyImages & P/G  \\
Plain & 93.20  & 49.9 & 0.0  & 93.7 & 0.0  & 98.9 & 0.0  & 97.3 & 0.0  & 87.5 & 0.0  & 90.0 & 0.0  \\
CEDA CE Uni & 90.80  & 50.0 & 0.0  & 90.0 & 0.0  & 100.0 & 0.0  & 94.4 & 0.0  & 85.1 & 0.0  & 87.5 & 0.0 \\
CEDA CE Tiny & 91.80  & 50.0 & 0.0  & 99.2 & 0.0  & 97.9 & 0.0  & 100.0 & 0.0  & 93.2 & 0.0  & 97.4 & 0.0  \\
Quantile 1.0 & 93.10  & 49.9 & 0.0  & 98.6 & 0.0  & 98.7 & 0.0  & 98.8 & 0.0  & 94.0 & 0.0  & 97.4 & 0.0  \\
Quantile 0.9 & 86.30  & 49.9 & 0.7  & 96.6 & 13.0  & 97.9 & 69.1  & 97.8 & 17.6  & 89.1 & 2.3  & 94.5 & 5.0  \\
Quantile 0.7 & 71.20  & 48.9 & 5.0  & 83.7 & 26.3  & 98.7 & 0.0  & 84.3 & 42.5  & 78.2 & 11.7  & 84.8 & 16.1  \\
Full ibp & 57.90  & 50.0 & 30.2  & 82.0 & 66.3  & 94.5 & 88.1  & 94.1 & 80.0  & 76.6 & 55.1  & 84.5 & 65.9  \\
\bottomrule
\end{tabularx}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

\begin{table*}[t]
\caption{eps=0.01. 20 steps. 1000 samples. all models RN20, eexcept CEDA CE Tiny which is RN32.}
\setlength\tabcolsep{.5pt} % default value: 6pt
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\makebox[\textwidth][c]{
\begin{tabularx}{1.3\textwidth}{lc|CC|CC|CC|CC|CC|CC|CC|CC|CC}
\toprule
Model & Acc. & CIFAR10 & P/A & SVHN & P/A & uniform & P/A & low freq & P/A & CIFAR100 & P/A & TinyImages & P/A  \\
Plain & 93.20  & 49.9 & 2.3  & 93.7 & 6.7  & 98.9 & 79.0  & 97.3 & 16.4  & 87.5 & 5.6  & 90.0 & 7.6  \\
CEDA CE Uni & 90.80  & 50.0 & 2.2  & 90.0 & 8.7  & 100.0 & 100.0  & 94.4 & 12.8  & 85.1 & 8.4  & 87.5 & 11.2 \\
CEDA CE Tiny & 91.80  & 50.0 & 4.0  & 99.2 & 13.3  & 97.9 & 64.0  & 100.0 & 41.6  & 93.2 & 16.2  & 97.4 &  24.5  \\
Quantile 1.0 & 93.10  & 49.9 & 2.2  & 98.6 & 82.2  & 98.7 & 94.8  & 98.8 & 98.5  & 94.0 & 49.2  & 97.4 & 77.8  \\
Quantile 0.9 & 86.30  & 49.9 & 9.7  & 96.6 & 70.8  & 97.9 & 97.9 & 97.8 & 95.1  & 89.1 & 45.6  & 94.5 & 66.3  \\
Quantile 0.7 & 71.20  & 48.9 & 23.9  & 83.7 & 74.2  & 98.7 & 95.7  & 84.3 & 80.1  & 78.2 & 53.4  & 84.8 & 65.3  \\
Full ibp & 57.90  & 50.0 & 39.2  & 82.0 & 74.7  & 94.5 & 93.7  & 94.1 & 88.9*  & 76.6 & 66.2  & 84.5 & 76.0  \\
\bottomrule
\end{tabularx}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


\begin{table*}[t]
\caption{MNIST eps=0.1. 10000 samples FMNIST, CIFAR10, UniformNoise, MNIST, 20800 EMNIST, 25000 TinyImages.}
\setlength\tabcolsep{.5pt} % default value: 6pt
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\makebox[\textwidth][c]{
\begin{tabularx}{1.3\textwidth}{lc|CC|CC|CC|CC|CC|CC|CC|CC|CC}
\toprule
Model & Acc. & FMNIST & P/G & Tiny & P/G & CIFAR10 & P/G & EMNIST & P/G & MNIST & P/G & Uniform & P/G & MIRROR & P/G  \\
Plain & 99.48  & 97.7 & 0.0  & 98.6 & 0.0  & 98.5 & 0.0  & 87.9 & 0.0  & 50.0 & 0.0  & 99.4 & 0.0  & 85.7 & 0.0  \\
CEDA LC Tiny & 99.46  & 100.0 & 0.0  & 100.0 & 0.0  & 100.0 & 0.0  & 92.8 & 0.0  & 50.0 & 0.0  & 100.0 & 0.0  & 85.9 & 0.0  \\
Quantile 0.2 & 98.62 & 99.8 & 90.5  & 100.0 & 99.5  & 100.0 & 100.0  & 98.3 & 47.0  & 50.0 & 0.3  & 100.0 & 100.0  & 84.3 & 0.9  \\
Quantile 0.0 & 97.11  & 100.0 & 99.8  & 100.0 & 99.7  & 100.0 & 100.0  & 98.9 & 71.3  & 50.0 & 1.0  & 100.0 & 100.0  & 82.3 & 4.8  \\
\bottomrule
%/mnt/SHARED/Julian/models_for_eval/provable_lc_MNIST/05-25-21-22-14lc_ibpLquantile_square_logit_spread0.0e0.5k0.3bs128ALwd0.05c4r0oTinyImagesm0.9Crop4/state_dicts/419fin.pt
%/mnt/SHARED/Julian/models_for_eval/provable_lc_MNIST/05-25-21-22-18lc_ibpLquantile_square_logit_spread0.2e0.5k0.3bs128ALwd0.05c4r0oTinyImagesm0.9Crop4/state_dicts/419fin.pt
%/mnt/SHARED/Julian/models_for_eval/provable_lc_MNIST/05-25-21-13-18lc_ibpLceda+e0.5k1.0bs128ALwd0.05c4r0oTinyImagesm0.9Crop4/state_dicts/419fin.pt
%/mnt/SHARED/Julian/models_for_eval/provable_lc_MNIST/05-25-18-03-35plainLlogit_spreade0.0k0.0bs128ALwd0.05c4r0oTinyImagesm0.9Crop4/state_dicts/419fin.pt
\end{tabularx}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> tables/table_schedules.tex <==
\newlength{\schedwidth}
\setlength{\schedwidth}{3cm}
\begin{table}[t]
\caption{Training schedules for $\epsilon$ and $\kappa$ over epochs.} 
\label{table:schedules}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cccc}
\toprule
 & $\epsilon$ & $\kappa$   \\
\midrule
\rotatebox[origin=c]{90}{\centering MNIST}  & \includegraphics[align=c, width=\schedwidth]{images/schedules/MNIST_eps.png} & \includegraphics[align=c, width=\schedwidth]{images/schedules/MNIST_kappa.png} \\
\midrule
\rotatebox[origin=c]{90}{CIFAR-10}   & \includegraphics[align=c, width=3.2cm]{images/schedules/C10_eps.png} & \includegraphics[align=c, width=3.4cm]{images/schedules/C10_kappa.png} \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

